Bivariate change point detection in movement direction and speed

Biological movement patterns can sometimes be quasi linear with abrupt changes in direction and speed, as in plastids in root cells investigated here. For the analysis of such changes we propose a new stochastic model for movement along linear structures. Maximum likelihood estimators are provided, and due to serial dependencies of increments, the classical MOSUM statistic is replaced by a moving kernel estimator. Convergence of the resulting difference process and strong consistency of the variance estimator are shown. We estimate the change points and propose a graphical technique to distinguish between change points in movement direction and speed.

==> Supplement1.tex <==


\section*{Supplement 1: Univariate change point detection}
	
	Here we shortly discuss problems and restrictions of the univariate moving window approach. As described there, we derive the process $(D_i)_i$ of differences of estimated directions according {to the following equation}
    \begin{equation}
        D_i:=D_i(\hat{\vartheta}_{\ell},\hat{\vartheta}_{r}):=
		\text{atan2}(\sin(\hat{\vartheta}_{r}-\hat{\vartheta}_{\ell}),\cos(\hat{\vartheta}_{r}-\hat{\vartheta}_{\ell})), \label{eq:mosum}
	\end{equation}
    and use its maximum, $M$, as a test statistic for the null hypothesis of no change in direction. In order to derive a rejection threshold for the statistical test, we need the distribution of $M$ under the null hypothesis. As it is not easily accessible formally, we simulate the distribution of $M$ by assuming that all other parameters, particularly $r$, are constant. The empirical $(1-\alpha)$-quantile of the resulting simulations then serves as rejection threshold, $Q$.
	
	Figure \ref{fig:uni5} A shows that for the used parameter sets, the chosen significance level can be kept in  this setting both for the RW and the LW already for a window size of $h=30$. However, one should note that for small sample sizes, the step length $r$ may tend to be overestimated. To see this, consider first the degenerate case with $r=0$ in which the distribution of increments is centered at the origin. The distribution of $\hat \mu$ is then also normal and centered at the origin. Thus, the true expectation of $r$ should be zero, but by construction, all estimates $\hat r$ are positive, such that $r$ must necessarily be overestimated. If the distribution of $\hat \mu$ is shifted only slightly away from zero, this effect will remain. It is therefore necessary to assume a sufficiently large value of $\frac{r}{\sigma}$ (Figure \ref{fig:uni5} F).
	
	
	
	\begin{figure}[!h]
		\centering
		\includegraphics[width=1\textwidth]{plot_paper_neues_format_plot4.pdf}
 		\caption{Empirical significance level (A) and test power (B) for the LW and RW for $\alpha=5\%$. $1000$ simulations were performed with $h=30,\vartheta=35^\circ$ and $T=400$, and $\sigma=0.5$ for the testpower. (C) Distribution of increments before (blue) and after (green) the change point. Estimated expectation from mixture of increments (orange) and the resulting estimated direction and step length. Local and global estimators of the model parameters step length $r$ (D) and $\sigma^2$ (E) with window size $h=30$ from a track with one change in direction. (F) Estimation of the step length $r$ from data without change points. Mean of estimated step length (green line) and true step length (orange line). 1000 Simulations per step length $r$, $\sigma^2=1$, $h=30.$ (G) Track from the Linear Walk model with one change point $cp_\vartheta$ in direction and one change point $cp_r$ in step length. (H) Process of $|D_t|$ of the absolute value of differences of directions (black) derived from the track in G, threshold $Q_{glob}$ derived from global estimation of step length (red). Thresholds $Q_{r_1}$ and $Q_{r_2}$ derived from estimations of step lengths on either side of the change point in step length (green). Threshold $Q_{r_1,r_2}$ derived from tracks with the change point in step length (blue).}	
		\label{fig:uni5}
	\end{figure}

	If we apply the global parameter estimates in cases with change points in the model parameters, we observe a certain bias both in the RW and in the LW case. If a track contains one change point in direction, the increments between successive points are assumed to originate from two different normal distributions with the same variance $\sigma^2$ and the same distance $r$ to the origin, but with different directions from the origin (Figure \ref{fig:uni5} C). In that case, the step length $r$ will tend to be underestimated (purple line in panel E), and the standard deviation $\sigma$ will tend to be overestimated  (purple line in panel D). 	We therefore propose to apply a moving window approach and to use the median of the resulting process as a parameter estimate 		(red dashed line in Figure \ref{fig:uni5} D and E). 
	
	
	In our simulations with change points, the test power increased with the difference in directions and with increasing step length. In addition, it was higher for the LW than for the RW (Figure \ref{fig:uni5} B) for the same parameters, which is due to a higher variability in the RW.
		
	This indicates that the proposed statistical tests are suitable for detecting changes in the movement direction under the assumption of constant step length. However, one should note that additional change points in $r$ as illustrated in Figure \ref{fig:uni5} G will affect the rejection threshold $Q$, because $Q$ depends on $r$ (Figure \ref{fig:uni5} H). Smaller values of $r$ yield a higher variability of $|D|$ and thus, a higher $Q$ (green lines in Figure \ref{fig:uni5} H). Ignoring potential changes in $r$, one will obtain a false global estimate of  $r$  (red line in Figure \ref{fig:uni5} H), such that the resulting global rejection threshold $Q_{glob}$ cannot adhere to the chosen significance level. % (Figure \ref{fig:uni5} D, red line).% If we knew the change points in the step length, we could simulate a valid threshold $Q_{r_1,r_2}$  (Figure \ref{fig:uni5} D, blue line). However, this would require the changes in $\vartheta$ to be known as the estimation of $r$ itself is affected by changes in the direction $\vartheta$. \kgs{Note: Figur anpassen und ggf kuerzen.}


==> Supplement2.tex <==
\section*{Supplement 2: Details of the Recording and Post-processing}\label{appendix:datarecording}
	
	\subsection*{Data Acquisition}\label{appendix:acquisition}
	
	The data for organelle tracking was generated via light sheet-based fluorescence microscopy of 10-day old \textit{Arabidopsis thaliana} roots. The sample holder technique proposed by \cite{Wangenheim2015} was basis for sample preparation. Accordingly, the plants needed to be grown under sterile conditions on solid nutrient medium in a $45^{\circ}$-tilted manner within glass cuvettes with a diameter of 3 mm.
	
	The time laps data was recorded using a monolithic digital scanning light sheet-based fluorescence microscope \cite{Keller2010} combined with an EC Plan Neofluar 5x/0.16 air (Zeiss) lens for illumination and a WN Achroplan 40x/0.75 W (Zeiss) objective for detection of the fluorescence. Excitation wave length of 488 nm and detection between 500 and 550 nm utilizing a bandpass filter 525/47 were applied to image GFP-fluorescence, while 561 nm excitation wave length and 607/70 bandpass filter were used to image mCherry-fluorescence. The exposure time of the laser was kept to 20 ms. The data was collected utilizing an EMCCD camera compiling a display window for the used objective of 224.46 $\mu$m x 168.7 $\mu$m, which is composed of 1392 x 1040 pixels, therefore the resolution is 0.16125 $\mu m$.
	
	To image living organelles in roots, fluorescent marker lines generated by tDNA insertion were used. To visualise plastids, the fluorescent marker protein GFP was fused to the plastid transport signal sequence (tp), which is used in nature to target the small subunit (SSU) of the protein Rubisco to the plastid (tpSSU-GFP). To fluorescently stain peroxisomes, the peroxisome targeting signal SKL was fused to the fluorescent marker mCherry (mCherry-SKL). Both plant lines were selected by BASTA resistance.
	
	Image data was acquired of both marker lines by imaging 30 $\mu$m deep into the mature zone of the root in 1 $\mu$m steps, resulting in a stack of 31 two-dimensional greyscale microscopy images. A stack was recorded each 4.3 seconds, for the plastid marker line over a time course of 1 h resulting in 841 timepoints, while the peroxisome marker line was recorded for 30 min generating a set of 421 time points.

 
	\subsection*{Detection and Tracking}
	
	\label{appendix:detectiontracking}
	
	Detection and tracking was done as follows. Peroxisome movement was tracked using the software Arivis Vision 4D Version 3.5.1. After converting the data into .sis format via the arivis SIS Converter, the data was first segmented to create digital objects for each peroxisome by using the implemented ''blob finder'' function. As settings for the blob finder for the peroxisome data a diameter  1.2 $\mu$m for tracking, a probability threshold of 20 \% and a split sensitivity of 70 \% for tracking were applied. The segmented objects were interconnected over each time point by hand, making use of the 3D viewer function of the software, gaining a table of the 3-dimensional coordinates of each peroxisome over time.\\
	
	Detection and tracking of the plastides was performed using the TrackMate Plugin (version=4.0.1) \citep{trackmate} of FIJI \cite{FIJI}. For the particle detection step the Laplacian of Gaussian Detector (LoG Detector) was used, which applies a Gaussian filter to the image and then uses the parameter "radius" to identify local maxima (light spots in front of darker background) as spots, we chose radius$=2\mu m$. Each spot has a quality value, which is a measure of how sure the algorithm is to have identified a ''True'' spot. Since we have a stack of microscopy images for each time point our spots are technically balls. After selecting a lower threshold for the quality parameter by visually checking the effect of different thresholds, the detection is executed on the image stack for each time point resulting in spacio-temporal coordinates (t,x,y,z) per detected spot.
	
	For the tracking the LAP Tracker (Linear Assignment Tracker) was used. This Tracker considers the spots from two consecutive time points $t$ and $t+1$. For each possible Spot pair $(s_t,s_{t+1})$ the Tracker assigns a cost value for linking based on the euclidean distance between the spots. Then the linking configuration with the minimum cost between the spots from time $t$ to $t+1$ is chosen. This is repeated for every consecutive time point pair, resulting in time series of spots. For a more detailed explanation of the algorithms as well as the usage of the software see the TrackMate entry of the FIJI website \cite{FIJI} and the documentation which can be found on the website.
	
	The settings used for detection and tracking in the TrackMate Plugin for Fiji (version 4.0.1) were as follows. For the LoG detector, median filtering was off, sub-pixel localisation was allowed, and we used values of radius of 2 $\mu m$, target channel of $1$ and a threshold of zero. For the spot filter collection, the quality was set to $\ge 18.2$ and the estimated diameter to $\ge 2.0 \mu m$. For the LAP tracker, track splitting and merging was not allowed, the maximal linking distance and gap closing distance were $15 \mu m$ and the maximum frame gap was $2$.		
	
	\subsection*{Post-Processing}
	
	\label{appendix:postprocessing}
	
	Since we obtained the plastid movement tracks by using automated tracking with the LAP-tracking algorithm from the TrackMate Plugin, which in general "rarely gives an error free result" \cite{Beltman2009}, we post-processed the tracks.
	
	First we made two quick adjustments to the data set. Since we are interested in the long-term behaviour of plastide movements, we chose to keep only tracks with recording times longer than 100 time points. Then we discarded tracks which contained so-called {border tracking}. {Border tracking} \cite{Beltman2009} occurs when cell organelles move outside the rectangular cuboid of the microscopy area. The position of a cell organelle is detected by finding its centre of mass, but since the fluorescence of the cell organelles slightly outside the microscopy area still spreads into it, their position will wrongly be detected as moving exactly in the border plane of the microscopy area. This leads to skewed results when characterizing the movement. Therefore, these tracks were discarded.
	
	The resulting tracks were individually analysed and corrected by hand due to smaller artefacts.  For every track $T$ we selected the set $S_T$ of all tracks observed within a certain small neighborhood of this track. We then investigated the 3D plot of these tracks as well as the process of their signal-to-noise ratios and step lengths between subsequent positions. We then performed three steps to eliminate three different artifacts. 
 
 First, the tracking algorithm globally minimizes the links between positions at time $t$ and $t+1$. If an organelle is  detected at time $t$ but not at time $t+1$, the algorithm may falsely assign another organelle to the same track, which may lead to isolated long jumps. If short peaks in the step length occurred when the plastide associated with the reference track was not detected, we separated the track and used the remaining parts individually if they were longer than 100 time points. 
 
Second, {track switching} (\cite{Beltman2009}) can occur when two plastides come into close proximity. The tracking algorithm, favouring short links, may then link the further movement of track $a$ with the start from track $b$, i.e. switching the first and second part of the two tracks. In our data, temporary close proximity of tracks was sometimes followed by a sudden switch in the level of the signal-to-noise ratios as well as a change in the step lengths. In these cases, we switched the tracks at the respective time. 
Third, double tracking (\cite{Beltman2009}) can occur when during spot detection the plastide, which can deform from vaguely spherical to stretched shape, was accidentally detected as two plastides. In our data set, some tracks suddenly stopped, where at the same time one of the near tracks started in very close proximity. If this occurred and if the signal-to-noise ratio and the step length of both tracks behaved  similarly, we connected the two tracks. This post-processing led to the final plastid data set of tracks used for analysis.


==> Supplement3.tex <==


\section*{Supplement 3: Unbiasedness of MLE based estimates from Proposition \textcolor{black}{2.2}}
	
	Here we show the unbiasedness of the estimators derived in Proposition \textcolor{black}{2.2}, which states that for a uni-directional \textbf{LW}($\vartheta$,$r$,$b$,$\sigma$,$\emptyset$) with a sequence of positions $X_{i+1}, X_{i+2}, \ldots, X_{i+h}$, the MLEs for $\mu$ and $\sigma^2$ are given, respectively, by 
		\begin{align}
			\hat{\mu}(i,h)&=\frac{6}{h^3-h}\sum_{j=1}^{\lfloor\frac{h}{2}\rfloor}\left(h-(2j-1)\right)\left(X_{i+j}-X_{i+h-j+1}\right), \label{eq:MLEmuLM}\\
			\hat{b}(i,h)  &= \bar X- (t+(h+1)/2)\hat\mu, \quad \text{and} \label{eq:MLEbLM}\\
			\hat{\sigma}^{2}(i,h) &=\frac{1}{2h}\sum_{j=1}^{h} \| X_{i+j}-(i+j)\hat\mu-\hat b\|^2,
			\label{eq:MLEsigmaLM}\end{align}
	where $\bar{X}:=h^{-1}\sum_{j=1}^h{X_{i+j}}$.
	
	We first note the following equalities for the weights in $\hat{\mu}^{(d)}$ and $\hat{b}^{(d)}$, which we denote by $w_\mu(h,j):=2j-h-1$ and $w_b(h,i,j):=-6hj-12ji-6j+4h^2+6hi+6h+6i+2$, respectively. Then we have
\begin{align}
		&\sum_{j=1}^{h}w_\mu(h,j)=0 \quad\text{ and }\quad \sum_{j=1}^{h}w_\mu(h,j)(i+j)=\frac{h^3-h}{6}, \label{eq:weightsumsmu}\\
		&\sum_{j=1}^{h}w_b(h,i,j)=h^3-h\quad \text{ and }\quad \sum_{j=1}^{h}w_b(h,i,j)(i+j)=0. \label{eq:weightsumsb}
	\end{align}
	
	We then find for $\hat{\mu}^{(d)}$
\begin{align*}
		\mathbb{E}\left[\hat{\mu}^{(d)}\right]&= \frac{6}{h^3-h}\sum_{j=1}^{h}w_\mu(h,j)\mathbb{E}\left[X_{i+j}^{(d)}\right]\\
		&=\frac{6}{h^3-h}\sum_{j=1}^{h}w_\mu(h,j)\left((i+j)\mu^{(d)}+b^{(d)}\right)\\
		&=\frac{6}{h^3-h}\left(\mu^{(d)}\sum_{j=1}^{h}w_\mu(h,j)(i+j) +b^{(d)}\sum_{j=1}^{h}w_\mu(h,j)\right)\\
		&=\frac{6}{h^3-h}\frac{h^3-h}{6}\mu^{(d)} = \mu^{(d)},
	\end{align*}
	where we use equation (\ref{eq:weightsumsmu}). For $\hat{b}^{(d)}$  we use equation (\ref{eq:weightsumsb}) and observe
\begin{align}
		\mathbb{E}\left[\hat{b}^{(d)}\right]&= \nonumber \frac{1}{h^3-h}\sum_{j=1}^{n}w_b(h,i,j)\mathbb{E}\left[X_{i+j}^{(d)}\right]\nonumber\\
		&= \frac{1}{h^3-h}\sum_{j=1}^{n}w_b(h,i,j) \left((i+j)\mu^{(d)}+b^{(d)}\right)\nonumber \\\
		&= \frac{1}{h^3-h}\left(\mu^{(d)}\sum_{j=1}^{n}w_b(h,i,j)(i+j)+b^{(d)}\sum_{j=1}^{n}w_b(h,i,j)\right) = b^{(d)}. \label{eq:b_unbiased}
	\end{align}
	%%%%%%%%%%%%%%%
    For the expectation of $\sigma^2$ we first insert equation \eqref{eq:MLEbLM} into equation \eqref{eq:MLEsigmaLM}, noting that
    \begin{align*}
        X_{i+j} -(i+j)\hat{\mu}-\hat{b} &= X_{i+j} - (i+j)\hat{\mu} - \bar{X} +\left(i+\frac{h+1}{2}\right)\hat{\mu}\\
        &= X_{i+j} - \bar{X} + \hat{\mu}\left( \frac{h+1}{2}-j \right).
    \end{align*}
    Now using $X_{i+j}=b+(i+j)\mu+b+\sigma Z_{i+j}$, we note that 
    \begin{align*}
        X_{i+j}-\bar{X} = \mu\left( j-\frac{h+1}{2}\right)+ \sigma\left(Z_{i+j}-\bar{Z} \right),
    \end{align*}
    where $\bar{Z}=\frac{1}{h}\sum_{j=1}^hZ_{j+i}$. For unbiasedness of $\hat{\sigma}^2$ we thus need to show that 
    \begin{align}
        \mathbb{E}\left[\sum_{j=1}^h \left\lVert\sigma\left( Z_{i+j}-\bar{Z}\right)+\left(\hat{\mu}-\mu\right)\left( \frac{h+1}{2}-j\right) \right\rVert^2  \right]= (2h-4)\sigma^2.\label{eq:hatsigmasquared_alternativeform}
    \end{align}
    The expression on the left of \eqref{eq:hatsigmasquared_alternativeform} equals $\sum_{j=1}^h\sum_{d=1,2}(a_1+a_2+a_3)$, with
    \begin{align*}
    a_1&= \sigma^2\mathbb{E}\left[\left( Z_{i+j}^{(d)}-\bar{Z}^{(d)}\right)^2\right],\\
    a_2&= 2\sigma\left( \frac{h+1}{2}-j\right)\mathbb{E}\left[\left(Z_{i+j}^{(d)}-\bar{Z}^{(d)}\right)\left(\hat{\mu}^{(d)}-\mu^{(d)}\right) \right],\\
    a_3&=\left( \frac{h+1}{2}-j\right)^2\mathbb{E}\left[\left(\hat{\mu}^{(d)}-\mu^{(d)}\right)^2\right].\label{eq:unbiasednesshatsigmasquared}
    \end{align*}
    We then observe
    \begin{align*}
        a_1&= \sigma^2\mathbb{E}\left[Z_{i+j}^{(d)^2}-2Z_{i+j}^{(d)}\bar{Z}^{(d)}+\bar{Z}^{(d)^2} \right]=\sigma^2\left(1-\frac{1}{h}\right),\\
        a_2 &= 2\sigma\left(\frac{h+1}{2}-j\right)\left(\mathbb{E}\left[Z_{i+j}^{(d)}\hat{\mu}^{(d)}\right] - \mathbb{E}\bigg[\bar{Z}^{(d)}\hat{\mu}^{(d)}\bigg] \right).
     \end{align*}
Now we note that
    \begin{align*}
        \mathbb{E}\left[Z_{i+j}^{(d)}\hat{\mu}^{(d)}\right]&= \mathbb{E}\left[Z_{i+j}^{(d)}\frac{6}{h^3-h}\sum_{k=1}^hw_\mu(h,k)X_{i+k}^{(d)}  \right]\\
        &=  \frac{6}{h^3-h}w_\mu(h,j)\mathbb{E}\left[Z_{i+j}^{(d)}X_{i+j}^{(d)}\right] \\
        &= \frac{6}{h^3-h}w_\mu(h,j)\mathbb{E}\left[Z_{i+j}^{(d)}(\mu^{(d)}+b^{(d)}+\sigma Z_{i+j}^{(d)})\right]\\
        &= \sigma \frac{6}{h^3-h}w_\mu(h,j)
    \end{align*}
    and
    \begin{align*}  \mathbb{E}\left[\bar{Z}^{(d)}\hat{\mu}^{(d)}\right] &= \mathbb{E}\left[\frac{1}{h}\sum_{k=1}^hZ_{i+k}^{(d)}\frac{6}{h^3-h}\sum_{l=1}^hw_\mu(h,l)X_{i+l}^{(d)}\right]\\
        &=\frac{6}{h(h^3-h)} \mathbb{E}\left[\sum_{k=1}^h\sum_{l=1}^hw_\mu(h,l)X_{i+l}^{(d)}Z_{i+k}^{(d)} \right]\\
        &= \frac{6}{h(h^3-h)} \left( \sum_{l=1}^h{w_\mu(h,l)\mathbb{E}\left[Z_{i+l}X_{i+l}\right]}  \right)\\
        &= \frac{6\sigma}{h(h^3-h)}{\sum_{l=1}^hw_\mu(h,l)}= 0
    \end{align*}
and hence find 
\begin{align*}
       a_2 &= 2\sigma\left(\frac{h+1}{2}-j\right)\left( \sigma\frac{6}{h^3-h}w_\mu(h,j) \right)
        =-\sigma^2\frac{6}{h^3-h}w_\mu(h,j)^2.
\end{align*}
For $a_3$ we have
    \begin{align*}
        a_3 
        &= \left(\frac{h+1}{2}-j\right)^2\left(\mathbb{E}\bigg[\hat{\mu}^{(d)^2}\bigg] -2\mu^{(d)}\mathbb{E}\bigg[\hat{\mu}^{(d)}\bigg] + \mu^{(d)^2}\right)
        =\frac{1}{4}\frac{12}{h^3-h}\sigma^2w_\mu(h,j)^2.
    \end{align*}
In total, the left hand side of \eqref{eq:hatsigmasquared_alternativeform} equals
    \begin{align*}
        \lefteqn{\sum_{j=1}^h\sum_{d=1,2}(a_1+a_2+a_3)}\\
        &=\sum_{j=1}^h\sum_{d=1,2} \left(\sigma^2\left(1-\frac{1}{h}\right) -\sigma^2\frac{6}{h^3-h}w_\mu(h,j)^2 + \frac{1}{4}\frac{12}{h^3-h}\sigma^2w_\mu(h,j)^2  \right)\\
        &= 2h\sigma^2\left(1-\frac{1}{h}\right)-2\sigma^2\frac{6}{h^3-h}{\sum_{j=1}^hw_\mu(h,j)^2}+2\sigma^2\frac{3}{h^3-h}\sum_{j=1}^hw_\mu(h,j)^2\\
        &=\left( 2(h-1)-\frac{12}{h^3-h}\frac{1}{3}(h^3-h)+\frac{6}{h^3-h}\frac{1}{3}(h^3-h) \right)\sigma^2\\
        &= (2h-4)\sigma^2,
    \end{align*}
    where we used that $\sum_{j=1}^hw_\mu(h,j)^2=(h^3-h)/3$.
	\qed



==> Supplement4.tex <==


\section*{Supplement 4: Strong Consistency of $\hat{b}^{(d)}$ and $\hat{\sigma}^2$}\label{supplement:strongconsistencysigmasquared}

The strong consistency of $\hat{b}^{(d)}$ can be shown using the SLLN for weighted sums from Proposition \textcolor{black}{B.1}. In the time continuous setting, $\hat{b}$ is given by
	\begin{align*}
		\hat{b}(nt,n\eta)&= \frac{1}{\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor}\sum_{j=1}^{\lfloor n\eta\rfloor}w_b(n\eta,nt,j)X^{(d)}_{\lfloor nt\rfloor+j}\\
		&= \sum_{j=1}^{\lfloor n\eta\rfloor}\frac{w_b(n\eta,nt,j)}{\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor}X^{(d)}_{\lfloor nt\rfloor+j}\\
        &= \sum_{j=1}^{\lfloor n\eta\rfloor}v(n,j)X^{(d)}_{\lfloor nt\rfloor+i}
	\end{align*}
	where we define 
    \begin{align*}
        \lefteqn{w_b(n\eta,nt,j):=}&\\
        &-6\lfloor n\eta\rfloor j-12j\lfloor nt\rfloor-6j+4\lfloor n\eta\rfloor^2+6\lfloor n\eta\rfloor \lfloor nt\rfloor+6\lfloor n\eta\rfloor+6\lfloor nt\rfloor+2
    \end{align*} and 
$v(n,j):=w_b(n\eta,nt,j)/(\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor)$.
    Again, using the arguments from Appendix \textcolor{black}{B}, it is sufficient to show that $\sum_{j=1}^{m(n)}v(n,j)^2 \in \mathrm{O}(n^{-1})$. This is the case because $w_b(n\eta,nt,j) \in \mathrm{O}(n^2)$ and thus,
	\begin{align*}
		\sum_{j=1}^{\lfloor n\eta\rfloor}v(n,j)^2 &= \underbrace{\frac{1}{(\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor)^2}}_{\in \mathrm{O}(n^{-6})}\underbrace{\sum_{j=1}^{\lfloor n\eta\rfloor}\underbrace{w_b(n\eta,nt,j)^2}_{\in \mathrm{O}(n^4)}}_{\in \mathrm{O}(n^{5})} \in \mathrm{O}(n^{-1}).
	\end{align*}       


    To prove strong consistency of $\hat{\sigma}^2$ we use the following variation of the SLLN in a setting of dependent, weighted sums.
    \begin{proposition}[SLLN with weights]\label{proposition:SLLNnew}\quad\\
		Let $X_{jk}$ be centred, i.e., $\mathbb{E}[X_{jk}]=0$, but not necessarily independent or identically distributed random variables with $\sup_{j\ge 1}\mathbb{E}[X_{jk}^6] < \infty$. Let \begin{equation*}S_n:= \sum_{j,k=1}^{m_n} v(n,j,k) X_{jk},\end{equation*} 
where $m_n\in\mathbb{N}$ and $v(n,j,k)\in\mathbb{R}$ are weights. Then $\lim\limits_{n\rightarrow\infty}S_n=0$ almost surely if the following term is in $\mathrm{O}(n^{-2})$
        \begin{align}
            &\sum_{i,j=1}^{m_n}v(n,i,j)^4 + \sum_{\substack{i,j,k,l=1\\ (i,j)\neq(k,l)}}^{m_n} v(n,i,j)^3v(n,k,l)\nonumber\\
            &+\sum_{\substack{i,j,k,l=1\\ (i,j)\neq(k,l)}}^{m_n}v(n,i,j)^2v(n,k,l)^2 +\nonumber\\
            &+\sum_{\substack{i,j,k,l,o,p=1\\ (i,j)\neq(k,l)\\ (i,j)\neq(o,p)\\ (o,p)\neq(k,l)}}^{m_n}v(n,i,j)v(n,k,l)v(n,o,p)^2\nonumber\\
            &+\sum_{\substack{i,j,k,l,o,p,r,s=1;\\ (i,j),(k,l),\\(o,p),(r,s)\\ \text{ pairwise different}}}^{m_n}v(n,i,j)v(n,k,l)v(n,o,p)v(n,r,s).\label{eq:langerterm}
        \end{align}
	\end{proposition}
Proposition \ref{proposition:SLLNnew} can be proven by a standard argument based on the Lemma of Borel--Cantelli and Markov's inequality.\\


Before we show strong consistency of $\hat{\sigma}^2$, we rewrite the estimator. For convenience, these calculations use the time discrete MLE for $\sigma^{2}$ as given in Proposition \textcolor{black}{2.2}. We first refer to a simpler notation of $\hat \sigma^2$ given in \textcolor{black}{(7) in Supplement 3}, i.e., 
    \begin{align}
        (2h-4)\hat\sigma^2 &=\sum_{j=1}^h \left\lVert\sigma\left( Z_{i+j}-\bar{Z}\right)+\left(\hat{\mu}-\mu\right)\left( \frac{h+1}{2}-j\right) \right\rVert^2
		\nonumber\\
  &=\sum_{j=1}^h \sum_{d=1,2}\left(\sigma\left( Z_{i+j}^{(d)}-\bar{Z}^{(d)}\right)+\left(\hat{\mu}^{(d)}-\mu^{(d)}\right)\left( \frac{h+1}{2}-j\right)\right)^2, \label{eq:hatsigmasquared_appendix}
	\end{align}
    where the superscript $(d)$ indicates the component of each vector in dimension $d$. For the second summand in the square we find
    \begin{align}
        \lefteqn{\left(\hat{\mu^{(d)}}-\mu^{(d)}\right)\left( \frac{h+1}{2}-j\right)}\nonumber\\ 
        &=\left(\frac{6}{h^3-h}\sum_{k=1}^hw_\mu(h,k)\left((i+k)\mu^{(d)}+b^{(d)}+\sigma Z_{i+k}^{(d)}\right)-\mu^{(d)}\right)\left(-\frac{1}{2}w_\mu(h,j)\right),\label{eq:54}
    \end{align}        
    where $w_{\mu}(h,j):=2j-h-1$. Using that $\sum_{k=1}^hw_\mu(h,k)(i+k)={(h^3-h)}/{6}$ and the notation 
    \begin{align*}
        \hat{\mu}^{(d)}(Z) = \frac{6}{h^3-h}\sum_{k=1}^{h}(2k-h-1)Z^{(d)}_{i+k},
    \end{align*} 
    the term in \eqref{eq:54} equals $-\frac{1}{2}w_\mu(h,j)\sigma \hat{\mu}^{(d)}(Z)$. Thus, we can rewrite $\hat \sigma^2$ as
	\begin{align}
		\hat{\sigma}^{2}(i,h)=\frac{\sigma^2}{2h-4}\sum_{j=1}^{h}\sum_{d=1,2}\left(Z^{(d)}_{i+j}-\bar{Z}^{(d)}-\frac{1}{2}w_{\mu}(h,j)\cdot \hat{\mu}^{(d)}(Z) \right)^2.\label{eq:sigmasimple}
	\end{align}
    Now we  show the strong consistency of $\hat{\sigma}^2(nt,n\eta)$, i.e., $\hat{\sigma}^{2}(nt,n\eta)-\sigma^2 \xrightarrow[n\rightarrow\infty]{}0$ almost surely, as stated in Proposition \textcolor{black}{3.1}, returning to the time continuous setting but making use of formula \eqref{eq:sigmasimple}. We start by rewriting $\hat\sigma^2$ into a sum of six summands for each dimension $d$.
    \begin{align}
        \lefteqn{\hat{\sigma}^{2}(nt,n\eta)}\nonumber\\
        &=\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}\sum_{j=1}^{\lfloor n\eta\rfloor}\sum_{d=1,2}\left(Z^{(d)}_{\lfloor nt\rfloor+j}-\bar{Z}^{(d)}-\frac{1}{2}w_{\mu}(n\eta,j)\cdot \hat{\mu}^{(d)}(Z) \right)^2\nonumber\\
		&=\sum_{d=1,2}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}\sum_{j=1}^{\lfloor n\eta\rfloor}\left(Z^{(d)^2}_{\lfloor nt\rfloor+j}+\bar{Z}^{(d)^2}+\left(\frac{1}{2}w_{\mu}(n\eta,j)\cdot \hat{\mu}^{(d)}(Z)\right)^2 \nonumber\\
		&\qquad~+2Z^{(d)}_{\lfloor nt\rfloor+j}\left(-\bar{Z}^{(d)}\right) +2Z^{(d)}_{\lfloor nt\rfloor+j}\left(-\frac{1}{2}w_{\mu}(n\eta,j)\cdot \hat{\mu}^{(d)}(Z)\right)\nonumber\\
        &\qquad~+2\left(-\bar{Z}^{(d)}\right)\left(-\frac{1}{2}w_{\mu}(n\eta,j)\cdot \hat{\mu}^{(d)}(Z)\right)  \bigg)\nonumber\\
		&=\sum_{d=1,2}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}\sum_{j=1}^{\lfloor n\eta\rfloor}\left(Z^{(d)^2}_{\lfloor nt\rfloor+j}+\bar{Z}^{(d)^2}+\frac{1}{4}w_{\mu}(n\eta,j)^2\hat{\mu}^{(d)}(Z)^2\nonumber\\
        &\qquad~-2Z^{(d)}_{\lfloor nt\rfloor+j}\bar{Z}^{(d)} -w_{\mu}(n\eta,j)Z^{(d)}_{\lfloor nt\rfloor+j}\hat{\mu}^{(d)}(Z) +w_{\mu}(n\eta,j)\bar{Z}^{(d)}\hat{\mu}^{(d)}(Z)  \bigg)\nonumber\\
		&=\sum_{d=1,2}\Bigg(\underbrace{\sum_{j=1}^{\lfloor n\eta\rfloor}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}Z^{(d)^2}_{\lfloor nt\rfloor+j}}_{=:S_1} +\underbrace{\sum_{j=1}^{\lfloor n\eta\rfloor}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}\bar{Z}^{(d)^2}}_{=:S_2}\nonumber\\
        &\qquad~+ \underbrace{\sum_{j=1}^{\lfloor n\eta\rfloor}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}\frac{1}{4}w_{\mu}(n\eta,j)^2\hat{\mu}^{(d)}(Z)^2}_{=:S_3}- \underbrace{\sum_{j=1}^{\lfloor n\eta\rfloor}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}2Z^{(d)}_{\lfloor nt\rfloor+j}\bar{Z}^{(d)}}_{=:S4}\nonumber\\
		&\qquad~ - \underbrace{\sum_{j=1}^{\lfloor n\eta\rfloor}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}w_{\mu}(n\eta,j)Z^{(d)}_{\lfloor nt\rfloor+j}\hat{\mu}^{(d)}(Z)}_{=:S_5}\nonumber\\
        &\qquad~+\underbrace{\sum_{j=1}^{\lfloor n\eta\rfloor}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}w_{\mu}(n\eta,j)\bar{Z}^{(d)}\hat{\mu}^{(d)}(Z)}_{=:S_6} \Bigg)\label{eq:hatsigmasquared_terms}
	\end{align}
	Since the summands in the two dimensions $d=1,2$ are independent, we focus on one dimension and suppress the index $d$. As $\hat{\sigma}^{2}(nt,n\eta)$ is unbiased we can split the expectation $\sigma^2$ into the expectations of each of the summands. We show that each summand in the brackets in \eqref{eq:hatsigmasquared_terms} centred with its expectation converges to $0$ almost surely.\\
	For summand 1 we have
	\begin{align*}
		S_1-\mathbb{E}[S_1] &= \sum_{j=1}^{\lfloor n\eta\rfloor}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}\left(Z^{(d)^2}_{\lfloor nt\rfloor+j} - \mathbb{E}\bigg[Z^{(d)^2}_{\lfloor nt\rfloor+j}\bigg]\right)\\
        &= \sum_{j=1}^{\lfloor n\eta\rfloor}v(n,j)\left(\underbrace{Z^{(d)^2}_{\lfloor nt\rfloor+j} - \mathbb{E}\bigg[Z^{(d)^2}_{\lfloor nt\rfloor+j}\bigg]}_{\mathbb{E}[*]=0}\right),
	\end{align*}
	where we here define $v(n,j):=\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}$. According to Proposition \textcolor{black}{ B.1}, we need to verify $\sum_{j=1}^{m_n}v(n,j)^2 \in \mathrm{O}(n^{-1})$. This holds because
	\begin{align*}
		\sum_{j=1}^{\lfloor n\eta\rfloor}v(n,j)^2 = \sum_{j=1}^{\lfloor n\eta\rfloor}\left(\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}\right)^2 = \sigma^4\frac{\lfloor n\eta\rfloor}{(2\lfloor n\eta\rfloor-4)^2} \in \mathrm{O}(n^{-1}).
	\end{align*}
	For summand 2, we use $\mathbb E \bar{Z}^{(d)^2} = 1/\lfloor n\eta\rfloor$ and get
	\begin{align*}
		S_2-{\mathbb{E}[S_2]} 
		&= \frac{\lfloor n\eta\rfloor \sigma^2}{2\lfloor n\eta\rfloor-4} \left(\bar{Z}^{(d)^2}-\mathbb E \bar{Z}^{(d)}^2\right)\\
        &= \frac{\lfloor n\eta\rfloor \sigma^2}{2\lfloor n\eta\rfloor-4} \bar{Z}^{(d)^2}-\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}\xrightarrow[n\rightarrow\infty]{}0 \text{ a.s.}
	\end{align*}
    For summand 3 we first rewrite $S_3$ as
	\begin{align*}
		S_3 
		&= \sum_{j=1}^{\lfloor n\eta\rfloor}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}\frac{1}{4}w_{\mu}(n\eta,j)^2\left(\frac{6}{\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor}\sum_{k=1}^{\lfloor n\eta\rfloor}w_{\mu}(n\eta,k)Z^{(d)}_{\lfloor nt\rfloor+k}\right)^2\\
%		&= \sum_{j=1}^{\lfloor n\eta\rfloor}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}\frac{1}{4}w_{\mu}(n\eta,j)^2 \frac{6^2}{(\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor)^2}\sum_{k,l=1}^{\lfloor n\eta\rfloor}w_{\mu}(n\eta,k)w_{\mu}(n\eta,l)Z^{(d)}_{\lfloor nt\rfloor+k}Z^{(d)}_{\lfloor nt\rfloor+l} - EW\\
		&= \sum_{k,l=1}^{\lfloor n\eta\rfloor}\underbrace{v(n,k,l)}_{\text{ in part 2 of Proposition \ref{proposition:SLLNnew}}}Z^{(d)}_{\lfloor nt\rfloor+k}Z^{(d)}_{\lfloor nt\rfloor+l},
	\end{align*}
    with 
    \begin{align*}
        v(n,k,l) := \frac{6^2\sigma^2}{4(2\lfloor n\eta\rfloor-4)(\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor)^2}\left(\sum_{j=1}^{\lfloor n\eta\rfloor}w_{\mu}(n\eta,j)^2\right) w_{\mu}(n\eta,k)w_{\mu}(n\eta,l)
    \end{align*}
    such that we have
    \begin{align*}
        S_3-\mathbb E [S_3] &= \sum_{k,l=1}^{\lfloor n\eta\rfloor}v(n,k,l)\left(Z^{(d)}_{\lfloor nt\rfloor+k}Z^{(d)}_{\lfloor nt\rfloor+l}-\mathbb E\left[Z^{(d)}_{\lfloor nt\rfloor+k}Z^{(d)}_{\lfloor nt\rfloor+l}\right]\right).
    \end{align*}
    To show almost sure convergence to $0$ we need to verify that the term in \eqref{eq:langerterm} is in $\mathrm{O}(n^{-2})$. We thus note that for the present definition of $v(n,k,l)$, the term in \eqref{eq:langerterm} corresponds to the following term
	\begin{align}
		  \lefteqn{\underbrace{\frac{6^8\sigma^8}{4^4(2\lfloor n\eta\rfloor-4)^4(\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor)^8}\left(\frac{\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor)}{3}\right)^4}_{\in \mathrm{O}(n^{-28}n^{12})=\mathrm{O}(n^{-16})}} \nonumber\\
		& ~\times \bigg[\underbrace{\sum_{j,k=1}^{\lfloor n\eta\rfloor}w_{\mu}(n\eta,j)^4w_{\mu}(n\eta,k)^4}_{\lfloor n\eta\rfloor^2\cdot \mathrm{O}(n^8)=\mathrm{O}(n^{10})}\nonumber\\
        & \qquad ~+\underbrace{\sum_{\substack{i,j,k,l=1\\ (i,j)\neq(k,l)}}^{\lfloor n\eta\rfloor}w_{\mu}(n\eta,i)^2w_{\mu}(n\eta,j)^2w_{\mu}(n\eta,k)^2w_{\mu}(n\eta,l)^2}_{\in\lfloor n\eta\rfloor^4\cdot \mathrm{O}(n^8)=\mathrm{O}(n^{12})}\nonumber\\
		& \qquad ~+ \underbrace{\sum_{\substack{i,j,k,l=1\\ (i,j)\neq(k,l)}}^{\lfloor n\eta\rfloor}w_{\mu}(n\eta,i)^3w_{\mu}(n\eta,j)^3w_{\mu}(n\eta,k)w_{\mu}(n\eta,l)}_{\in \lfloor n\eta\rfloor^4\cdot \mathrm{O}(n^8)=\mathrm{O}(n^{12})}\nonumber\\
		& \qquad ~+  \underbrace{\sum_{\substack{i,j,k,l,o,p=1\\ (i,j)\neq(k,l)\\ (i,j)\neq(o,p)\\ (o,p)\neq(k,l)}}^{\lfloor n\eta\rfloor} w_{\mu}(n\eta,i)w_{\mu}(n\eta,j)w_{\mu}(n\eta,k)w_{\mu}(n\eta,l)w_{\mu}(n\eta,o)^2w_{\mu}(n\eta,p)^2}_{\in\lfloor n\eta\rfloor^6\cdot \mathrm{O}(n^8)=\mathrm{O}(n^{14})}\nonumber\\
		& \qquad ~+  \sum_{\substack{i,j,k,l,o,p,r,s=1;\\ (i,j),(k,l),\\(o,p),(r,s)\\ \text{ pairwise different}}}^{\lfloor n\eta\rfloor} \prod_{q=i,j,k,l,o,p,r,s}w_{\mu}(n\eta,q)\bigg]\label{eq:langerterm_summand3}.%\\
%		&\in \mathrm{O}\left(\frac{n^{14}}{n^{16}}\right) =\mathrm{O}\left(n^{-2}\right)\nonumber
\end{align}
All sums in the latter display except for the last one are easily upper bounded and seen to be in $\mathrm{O}(n^{14}/n^{16})=\mathrm{O}\left(n^{-2}\right)$. The last sum requires an exact, tedious calculation. We used the Python module Sympy and obtained  $\mathrm{O}(n^{12}/n^{16})$.


For summand 4 we use  $\mathbb{E}[Z^{(d)}_{\lfloor nt\rfloor+i}\bar{Z}] = 1/\lfloor n\eta\rfloor$ and get
	\begin{align}
		S_4 - \mathbb{E}[S_4] 
		&= \sum_{j=1}^{\lfloor n\eta\rfloor}\frac{\sigma^2}{\lfloor n\eta\rfloor-2}\left(Z^{(d)}_{\lfloor nt\rfloor+j}\bar{Z}^{(d)} - \frac{1}{\lfloor n\eta\rfloor}\right) \xrightarrow[n\rightarrow\infty]{}0\label{eq:consistencyhatvariance_summand4}
	\end{align}
by the conventional SLLN. 
 
For summand 5 we again first rewrite $S_5$ as
	\begin{align*}
	S_5 
		&= \sum_{i=1}^{\lfloor n\eta\rfloor}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}w_{\mu}(n\eta,i)Z^{(d)}_{\lfloor nt\rfloor+i}\left(\frac{6}{\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor}\sum_{j=1}^{\lfloor n\eta\rfloor}w_{\mu}( n\eta,j)Z^{(d)}_{\lfloor nt\rfloor+j}\right),
  \end{align*}
  which yields
\begin{align*}
		S_5-\mathbb E[S_5]&= \sum_{i,j=1}^{\lfloor n\eta\rfloor} v(n,i,j)\left(Z^{(d)}_{\lfloor nt\rfloor+i}Z^{(d)}_{\lfloor nt\rfloor+j}- \mathbb E \left[Z^{(d)}_{\lfloor nt\rfloor+i}Z^{(d)}_{\lfloor nt\rfloor+j}\right]\right)
	\end{align*}
	where we define 
    \begin{align*}
        v(n,i,j):=\frac{6\sigma^2}{(2\lfloor n\eta\rfloor-4)(\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor)}w_{\mu}(n\eta,i)w_{\mu}(n\eta,j).
    \end{align*} 
    Now we are in the setting of the SLLN as in Proposition \ref{proposition:SLLNnew}, part 2 because the summands are not necessarily independent. Therefore we need to verify that the term in \eqref{eq:langerterm} is in $\mathrm{O}(n^{-2})$. We define the expression in the square brackets in \eqref{eq:langerterm_summand3} as $L$, for which we showed $L\in \mathrm{O}(n^{14})$ and find that the term in \eqref{eq:langerterm} in the current setting can be written as
	\begin{align*}
		\underbrace{\frac{6^4\sigma^8}{(2\lfloor n\eta\rfloor-4)^4(\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor)^4}}_{\in \mathrm{O}(n^{-16})}\cdot \underbrace{L}_{\in \mathrm{O}(n^{14})}\in \mathrm{O}(n^{-2}).
	\end{align*}
For summand 6 we first observe that 
\begin{align}
		\mathbb{E}\bigg[\bar{Z}^{(d)}\hat{\mu}^{(d)}(Z) \bigg] 
		&= \frac{6}{\lfloor n\eta\rfloor(\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor)}\sum_{k=1}^{\lfloor n\eta\rfloor}w_{\mu}(n\eta,k)\underbrace{\mathbb{E}\bigg[Z^{(d)^2}_{\lfloor nt\rfloor+k}\bigg]}_{=1}\nonumber\\
        &= \frac{6}{\lfloor n\eta\rfloor(\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor)}\underbrace{\sum_{k=1}^{\lfloor n\eta\rfloor}w_{\mu}(n\eta,k)}_{=0}=0, \label{eq:expectationnebenrechnung}
	\end{align}
such that	
\begin{align*}
		{S_6 - \mathbb{E}[S_6]}
		= \sum_{i=1}^{\lfloor n\eta\rfloor}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}w_{\mu}(n\eta,i)\bar{Z}^{(d)}\hat{\mu}^{(d)}(Z)
  %\\
	%	&= \sum_{i=1}^{\lfloor n\eta\rfloor}\frac{\sigma^2}{2\lfloor n\eta\rfloor-4}w_{\mu}(n\eta,i)\left(\frac{1}{\lfloor n\eta\rfloor}\sum_{j=1}^{\lfloor n\eta\rfloor}Z^{(d)}_{\lfloor nt\rfloor+j}\right)\left(\frac{6}{\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor}\sum_{k=1}^{\lfloor n\eta\rfloor}w_{\mu}(n\eta,k)Z^{(d)}_{\lfloor nt\rfloor+k}\right)\\
 	\end{align*}
This term vanishes because 
  \begin{align*}
\sum_{i=1}^{\lfloor n\eta\rfloor}w_{\mu}(n\eta,i) = 0.
  \end{align*}
 % &= \sum_{j,k=1}^{\lfloor n\eta\rfloor}\underbrace{\left(\sum_{i=1}^{\lfloor n\eta\rfloor}w_{\mu}(n\eta,i)\right)}_{=0}\frac{6\sigma^2}{(2\lfloor n\eta\rfloor-4)(\lfloor n\eta\rfloor^3-\lfloor n\eta\rfloor)\lfloor n\eta\rfloor}w_{\mu}(n\eta,k)Z^{(d)}_{\lfloor nt\rfloor+k}Z^{(d)}_{\lfloor nt\rfloor+j}\\
	
In total, each summand of $\hat{\sigma}^2(nt,n\eta)-\sigma^2$ converges to $0$ almost surely, which implies
	\begin{align*}
		\hat{\sigma}^{2}(nt,n\eta) \xrightarrow[n\rightarrow\infty]{} \sigma^{2} \text{   a.s.}
	\end{align*}



